Exploiting Structure for Optimal Multi-Agent Bayesian Decentralized Estimation

A key challenge in Bayesian decentralized data fusion is the `rumor propagation' or `double counting' phenomenon, where previously sent data circulates back to its sender. It is often addressed by approximate methods like covariance intersection (CI) which takes a weighted average of the estimates to compute the bound. The problem is that this bound is not tight, i.e. the estimate is often over-conservative. In this paper, we show that by exploiting the probabilistic independence structure in multi-agent decentralized fusion problems a tighter bound can be found using (i) an expansion to the CI algorithm that uses multiple (non-monolithic) weighting factors instead of one (monolithic) factor in the original CI and (ii) a general optimization scheme that is able to compute optimal bounds and fully exploit an arbitrary dependency structure. We compare our methods and show that on a simple problem, they converge to the same solution. We then test our new non-monolithic CI algorithm on a large-scale target tracking simulation and show that it achieves a tighter bound and a more accurate estimate compared to the original monolithic CI.

==> Figures/network_cGPT.tex <==
% \begin{figure}[tb]
% \centering
% \scalebox{0.5}{}{%
% \resizebox{1.6in}{2.55in}{
\begin{tikzpicture}[node distance=1.0cm, every node/.style={ draw=none, minimum size=0.7cm}]
  % First Row
  \node (1) {1};
  \node (2) [right of=1] {2};
  \node (3) [right of=2] {3};
  \node (4) [right of=3] {4};
  % \node (a) [above of=1, yshift=-0.4cm] {$(a)$};

  % Second Row
  \node (5) [below of=1] {5};
  \node (6) [right of=5] {6};
  \node (7) [right of=6] {7};
  \node (8) [right of=7] {8};

  % Third Row
  \node (10) [below of=6] {10};
  \node (9) [left of=10] {9};
  \node (11) [right of=10] {11};
  \node (12) [right of=11] {12};

  % Fourth Row
  \node (13) [below of=9] {13};
  \node (14) [right of=13] {14};
  \node (15) [below of=11] {15};
  \node (16) [below of=12] {16};

  % Edges
  \draw (4) -- (3);
  \draw (3) -- (2);
  \draw (2) -- (1);
  \draw (1) -- (2);
  \draw (1) -- (5);
  \draw (5) -- (6);
  \draw (6) -- (7);
  \draw (7) -- (8);
  \draw (7) -- (10);
  \draw (7) -- (11);
  \draw (11) -- (12);
  \draw (8) -- (12);
  \draw (12) -- (16);
  \draw (11) -- (15);
  \draw (10) -- (9);
  \draw (9) -- (13);
  \draw (9) -- (14);


  \begin{pgfonlayer}{background}
	% First rectangle
	\draw[fill=blue!10,rounded corners] (-0.3,0.35) rectangle (3.4,-0.25);
    \draw[fill=green!10,rounded corners] (-0.3,-0.7) rectangle (3.4,-1.3);
    \draw[fill=red!20,rounded corners] (-0.3,-1.7) rectangle (3.4,-2.3);
    \draw[fill=orange!10,rounded corners] (-0.3,-2.7) rectangle (3.4,-3.3);
	
     \end{pgfonlayer}
    \begin{scope}[node distance=1.0cm, every node/.style={ draw=none, minimum size=0.7cm}]
      % First Row
    \node (1) at (4.5,0) {1};
    \node (2) [right of=1] {2};
    \node (3) [right of=2] {3};
    \node (4) [right of=3] {4};
    % \node (b) [above of=1, yshift=-0.4cm] {$(b)$};

    \node (T1) at (4.1,-2.0) {$T_1$};
    \node (T2) [right of=T1] {$T_2$};
    \node (T3) [right of=T2] {$T_3$};
    \node (T4) [right of=T3] {$T_4$};
    \node (T5) [right of=T4] {$T_5$};
  

    % Edges
    \draw (4) -- (3);
    \draw (3) -- (2);
    \draw (2) -- (1);
    \draw (1) -- (2);

    \draw[-latex] (1) -- (T1);
    \draw[-latex] (1) -- (T2);
    \draw[-latex] (2) -- (T2);
    \draw[-latex] (2) -- (T3);
    \draw[-latex] (3) -- (T3);
    \draw[-latex] (3) -- (T4);
    \draw[-latex] (3) -- (T5);
    \draw[-latex] (4) -- (T4);
    \draw[-latex] (4) -- (T5);
    


  \begin{pgfonlayer}{background}
	% First rectangle
    \draw[fill=blue!10,rounded corners] (4.2,0.35) rectangle (7.8,-0.25);

    
	
     \end{pgfonlayer}

    \end{scope}
  
\end{tikzpicture}
 % }


 
  
% }

% \caption{Left: Undirected and cyclic network topology, split into 4 groups of 4 agents. Right: Target ($T_t$) tracking assignments to robots 1--4, other groups follow the same pattern. }
% \label{fig:net_topology}

% \vspace{-0.2in}

% \end{figure}


==> Text/0_Outline.tex <==
\begin{itemize}
    \item \textbf{Introduction:}
    \begin{itemize}
        \item DDF
        \item CI and conservatives
        \item approaches to reduce conservativeness - what's been done - split CI, Jiri Ajgl \cite{ajgl_rectification_2019}, safe fusion, etc.
        \item What we think can be done - 1. using optimization, 2. exploiting dependency structure. 
    \end{itemize} 
    \item \textbf{Problem statement:}
    \begin{itemize}
        \item DDF (homogeneous)  + searching for a tight bound on the fused result
        \item Description of the optimization problem.
    \end{itemize}
    \item \textbf{Technical approach:}
    \begin{itemize}
        \item Non-monolithic CI
        \item optimization
    \end{itemize}
    \item \textbf{Analysis/discussion:}
    \begin{itemize}
        \item Insigths from $1D$ and $2D$ solutions:$1D$ analytical solution.
        \item Can we narrow/limit the admissible correlations space? 
        \item Did anyone look at it from this angle?
        \item Can we find a ``worst-case" cross-correlation?  
        \item Compare nmCI to optimization solution. 
    \end{itemize}
    \item \textbf{Results/examples:}
    \begin{itemize}
        \item \textbf{So what?} Show what can we gain through simulations - Target tracking with independent directions? Explore different scale problems, compare RMSE, compare KLD?
        \item Otherwise- is it enough, for now, to compare nmCI and optimization solutions for $n>2$?
        \item Using optimization, can we prove/show that:\\
        1. nmCI is the \textbf{optimal solution} given the independence structure? \\
        2. nmCI is conservative? 
        \item What kind of assumptions/approximations can be done to enforce independence? Is it better than just using Vanilla CI?
    \end{itemize}
    
    \item Future work and summary
\end{itemize}
